NeuMap: Neural Coordinate Mapping by Auto-Transdecoder for Camera Localization

This paper presents an end-to-end neural mapping method for camera localization, dubbed NeuMap, encoding a whole scene into a grid of latent codes, with which a Transformer-based auto-decoder regresses 3D coordinates of query pixels. State-of-the-art feature matching methods require each scene to be stored as a 3D point cloud with per-point features, consuming several gigabytes of storage per scene. While compression is possible, performance drops significantly at high compression rates. Conversely, coordinate regression methods achieve high compression by storing scene information in a neural network but suffer from reduced robustness. NeuMap combines the advantages of both approaches by utilizing 1) learnable latent codes for efficient scene representation and 2) a scene-agnostic Transformer-based auto-decoder to infer coordinates for query pixels. This scene-agnostic network design learns robust matching priors from large-scale data and enables rapid optimization of codes for new scenes while keeping the network weights fixed. Extensive evaluations on five benchmarks show that NeuMap significantly outperforms other coordinate regression methods and achieves comparable performance to feature matching methods while requiring a much smaller scene representation size. For example, NeuMap achieves 39.1% accuracy in the Aachen night benchmark with only 6MB of data, whereas alternative methods require 100MB or several gigabytes and fail completely under high compression settings. The codes are available at https://github.com/Tangshitao/NeuMap

==> tex_file/1_introduction_old.tex <==
\section{Introduction}

Visual localization solves the camera position and orientation from its image observations, which is essential for applications including VR/AR and self-driving cars. Despite the rapid progress in this direction, accurate visual localization is still a challenging problem, especially when dealing with large viewpoint and illumination changes. Compact map representation is another increasingly important problem for visual localization. Applications such as delivering robots might need a map of every building and street corner of a big metropolitan area. Standard visual localization techniques require a massive database of key-points with 3D coordinates and visual features to be stored in or transferred to mobile agents, which becomes a significant bottleneck in real applications.


Most visual localization techniques first establish 2D-3D correspondences, and then estimate camera poses by perspective-n-point (PnP) ~\cite{lepetit2009epnp} with a sampling method such as RANSAC~\cite{fischler1981random}. These methods can be broadly divided into two categories. The first class is Feature Matching (FM)~\cite{sarlin2019coarse, sattler2012improving, cheng2019cascaded, yang2022scenesqueezer}, where some sparse robust features are extracted from the query image and matched with those in candidate scene images chosen by image retrieval techniques~\cite{arandjelovic2016netvlad, revaud2019learning}. By focusing on a sparse set of the most reliable points, this approach can exploit learning-based features extraction and correspondence matching methods~\cite{detone2018superpoint, sarlin2020superglue, sun2021loftr, tang2022quadtree}, which are trained with numerous image pairs of various view and illumination differences, to achieve robust localization. 
However, FM methods require a large map, i.e., a database of features with associated scene coordinates, which is impractical for large-scale scenes. Many methods~\cite{yang2022scenesqueezer, cheng2019cascaded, mera2020efficient} have been proposed to compress this map representation, but often at the cost of degraded performance.

The second class is Scene Coordinate Regression~(SCR)~\cite{brachmann2017dsac, brachmann2019expert, shotton2013scene, brachmann2021visual}, which uses a compact random forest or neural network to directly regress a dense scene coordinate map of the input image. These approaches train one model for each scene in a scene specific manner and achieve highly accurate results, but are often restricted to small-scale indoor scenes and limited viewpoint and illumination changes because the compact model has limited generalization capability. While ESAC~\cite{brachmann2019expert} can work with larger scenes by dividing them into smaller sub-regions, it still cannot handle large viewpoint and illumination changes.

We design our method to enjoy the benefits of compact scene representation of SCR methods and the robust performance of FM methods. Similar to FM methods, we also focus on a sparse set of robustly learned features to deal with large viewpoint and illumination changes. On the other hand, we exploit similar ideas to SCR methods to regress the 3D scene coordinates of these sparse features in the query images with a compact map representation. Our method, dubbed neural coordinate mapping (NeuMap), first extracts robust features from images and then applies a transformer-based auto-decoder (i.e., auto-transdecoder) to learn: 1) a grid of scene codes encoding the scene information (including 3D scene coordinates and feature information) and 2) the mapping from query image feature points to 3D scene coordinates. At test time, given a query image, after extracting image features of its key-points, the auto-transdecoder regresses their 3D coordinates via cross attention between image features and latent codes.
In our method, the robust feature extractor and the auto-transdecoder are scene-agnostic, where only latent codes are scene specific. This design enables the scene-agnostic parameters to learn matching priors across scenes while maintaining a small data size. To handle large scenes, we divide the scene into smaller sub-regions and process them independently while applying a network pruning technique~\cite{liu2017learning} to drop redundant codes.

We demonstrate the effectiveness of NeuMap with a diverse set of five benchmarks, ranging from indoor to outdoor and small to large-scale: 7scenes (indoor small), ScanNet (indoor small), Cambridge Landmarks (outdoor small), Aachen Day $\&$ Night (outdoor large), and NAVER LABS (indoor large). In small-scale datasets (i.e., 7scenes and Cambridge Landmarks), NeuMap compresses the scene representation by around 100-1000 times without any performance drop compared to DSAC++. In large-scale datasets (i.e., Aachen Day $\&$ Night and NAVER LABS), NeuMap significantly outperforms the current state-of-the-art at high compression settings, namely, HLoc~\cite{sarlin2019coarse} with a scene-compression technique~\cite{yang2022scenesqueezer}. In ScanNet dataset, we demonstrate the quick fine-tuning experiments, where we only optimize the codes for a new scene while fixing the scene-agnostic network weights. 


==> tex_file/2_relatedwork_old.tex <==
\section{Related work} 

\paragraph{Visual localization with feature matching (FM)} 
FM-based localization has achieved state-of-the-art performance.~\cite{sarlin2019coarse, sarlin2020superglue, detone2018superpoint, sattler2012improving, sun2021loftr, dusmanu2019d2, yang2022scenesqueezer, revaud2019r2d2}. Torsten et al. \cite{sattler2012improving} exhaustively match query images with all the 3D points in structure-from-motion models.
%and camera poses can be recovered from those 2D-3D correspondences. 
However, as the scene becomes large, this matching becomes ambiguous, impairing the robustness of the localization. Paul-Edouard~\cite{sarlin2020superglue} proposes a coarse-to-fine strategy: 1) Coarsely localizing the query images by a global image feature~\cite{arandjelovic2016netvlad}, and 2) Computing the camera poses by local key-point matches. This pipeline demonstrates significant improvements, where most follow-up works leverage the same pipeline and aim to improve the feature matching capability~\cite{yang2022scenesqueezer, sarlin2020superglue, sun2021loftr}. SuperGlue~\cite{sarlin2020superglue} learns to match two sets of key-points by Transformer, achieving impressive performance. Following superglue, LoFTR~\cite{sun2021loftr} and its variants~\cite{tang2022quadtree,chen2022aspanformer} propose a dense matching framework without the use of key-points. However, all those methods need to store a large database of key-point features or images. SceneSqueezer provides a compression mechanism to FM-based methods by removing redundant images and key-points, but their performance drop is significant at high compression settings. Our approach uses latent codes to store and retrieve key-point information, which naturally achieves high compression rates.

\paragraph{Scene coordinate regression (SCR)} 
Convolutional neural networks regress dense coordinate maps from RGB images for localization~\cite{brachmann2017dsac, brachmann2019neural, brachmann2021visual, brachmann2019expert, li2020hierarchical}. Due to the limited network capacity, The approach does not scale to large scenes.
For scalability, ESAC~\cite{brachmann2019expert} divides a large scene into smaller sub-regions and trains a network for each sub-region. HSCNet~\cite{li2020hierarchical} classifies a pixel into the corresponding sub-regions to reduce ambiguity. Although the representation size is smaller than FM-based methods, SCR-based methods are not robust against large viewpoint changes or illumination differences. The reason is that the acquisition of SCR training data is expensive (e.g., digital-cloning a city in different seasons at different times of day). On the other hand, FM training data is easily accessible where an extensive database of feature correspondences exists in challenging conditions~\cite{dai2017scannet, li2018megadepth}. Furthermore, this approach also requires model training for each novel scene, which is undesirable in applications. While SANet~\cite{yang2019sanet} and DSM~\cite{tang2021learning} generalize this approach to deal with unseen scenes, they also lead to reduced localization accuracy.   Our approach is SCR-based while utilizing a scene-agnostic feature extractor and transformer trained as in FM-based methods, which gives us both robustness and compact representation.


\paragraph{Auto-decoder} 
An auto-decoder directly optimizes a latent code via back-propagation with a decoder-only framework~\cite{park2019deepsdf, bojanowski2017optimizing, sitzmann2019scene}. Piotr et al.~\cite{park2019deepsdf} uses an auto-decoder for generative adversarial networks. DeepSDF~\cite{bojanowski2017optimizing} and SRN~\cite{sitzmann2019scene} store a shape representation into latent codes. However, MLP or CNN-based auto-decoder has limited capacity using a single code. Transformer-based autodecoder (i.e., auto-transdecoder) leverages an arbitrary number of codes to increase the capacity. Recently, Sandler et al.~\cite{sandler2022fine} augment a transformer with learnable memory tokens (codes) that allow the model to adapt to new tasks while optionally preserving its capabilities on previously learned tasks. The transformer weights are first pretrained with a large-scale dataset, while those tokens (codes) are then finetuned in downstream tasks. This memory mechanism is similar to our auto-transdecoder, while we optimize both transformer and codes simultaneously at the training time. To the best of our knowledge, this work is the first to use auto-transdecoder for mapping and localization tasks.



==> tex_file/3_method_OLD.tex <==
\input{fig/main_fig.tex}

% \section{Neural Coordinate Mapping}
\section{Method}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Structure of section 3
%[ intro blah blah ]
%We divide a scene into sub-regions. We will encode a scene information into a grid of codes over the sub-regions (in fact multiple codes per sub-region for expressiveness).
%We will explain data-preparation, architecture details, the training process, and the testing process.

%[ data preparation ]
%How to divide a scene into sub-regions.
%For each sub-region, we collect images, in-region points, and out-region points. We inject the information of points (3D coordinates and visual descriptors) and their in-region scores into codes.

%[ NeuMap architecture ]
%same as now.

%[ triaing ]
%same as now.

%[ testing ]
%K-image retrieval is a test-time process to me. That is a way to speed up the test-time process.
%ransac is also here, and how to combine multiple results from multiple sub-regions is another in this sub-section
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\I}{\mathbf{I}}
\newcommand{\iImages}{i}
\newcommand{\nImages}{N}
\newcommand{\qImage}{Q}
\newcommand{\qCamera}{C}
\newcommand{\coordFrame}{\mathcal{W}}
\newcommand{\keypoints}{P}
\newcommand{\keypoint}{\mathbf{k}}
\newcommand{\iKeypoints}{k}
\newcommand{\nKeypoints}{K}
\newcommand{\pixel}{\mathbf{p}}
\newcommand{\position}{\mathbf{x}}
\newcommand{\gridEdgeLength}{l}
\newcommand{\keypointExtractor}{\mathcal{K}}
\newcommand{\feature}{\mathbf{f}}
\newcommand{\Feature}{\mathbf{F}}
\newcommand{\voxel}{\mathcal{V}}
\newcommand{\voxCenter}{\mathbf{v}}
\newcommand{\tokens}{\mathbf{T}}
\newcommand{\token}{\mathbf{t}}
\newcommand{\iTokens}{t}
\newcommand{\nTokens}{T}
\newcommand{\confidence}{c}
\newcommand{\decoder}{\mathcal{D}}
\newcommand{\pars}{\boldsymbol{\theta}}
\newcommand{\scene}{\mathcal{S}}
\newcommand{\iScenes}{s}
\newcommand{\iVoxel}{v}
\newcommand{\proj}{\pi}
\newcommand{\hyper}{\lambda}
\newcommand{\W}{\mathbf{W}}

% \newpage
\TODO{Yasu, PTAL before it's baked-in}

\paragraph{Data preparation}
\begin{align}
\{\tilde\keypoint^\iKeypoints \in \real^2\} &= \keypointExtractor_\text{2D}(\I), \quad \forall \I \in \{\I_\iImages\}
&\text{(r2d2)}
\\
\{\keypoint^k \in \real^3\} &= \keypointExtractor_\text{3D}(\{\tilde\keypoint^k\}, \{\I_\iImages\})
&\text{(COLMAP)}
\\
(\feature^\iKeypoints_\iImages \in \real^D) &= \mathbf{F}_\iImages[\proj_\iImages(\keypoint^\iKeypoints) ] , \:\: \mathbf{F}_\iImages = \mathcal{E}(\I_\iImages)
&\text{(featurize)}
\end{align}

\paragraph{Factorization}
\begin{align}
\{\voxCenter_v\} &= \{ ( \mathbf{z} \odot \gridEdgeLength) \text{~~s.t.~~} \mathbf{z} \in \mathbb{Z}^3\}
&\text{(lattice)}
\\
\voxel_v &= \{ \keypoint^k \text{~s.t.~} \| \voxCenter_v - \keypoint^k \|_\infty \leq \gridEdgeLength \} 
&\text{(voxelize)}
\\
\mathcal{V} &= \{ \mathcal{V}_\iVoxel \text{~s.t.~} \mathcal{V}_v \neq \emptyset \} 
&\text{(sparsify)}
\end{align}

\paragraph{Prediction}
Given any pixel $\pixel \in [0,1]^2$ of a query image $\I$:
\begin{align}
\feature &= \Feature[\pixel], \:\: \Feature = \mathcal{E}(\I)
&\text{(pixel feature)}
\\
\mathcal{S} &= \{ \tokens_v \}, \:\: \tokens_v = \{\token_v^{(\iTokens)}\}_{\iTokens=1}^{\nTokens}
&\text{(scene tokens)}
\\
\position_v, \confidence_v &= \decoder(\feature; \tokens_v, \pars_\decoder)
&\text{(voxel decoder)}
\label{eq:decoder}
\end{align}

\paragraph{Decoder architecture}
The architecture of our decoder~$\decoder(\feature; \{\token^{(t)}\}, \pars_\decoder)$ is encoded by an inductive relationship starting from $\feature^{(1)}{=}\feature$; see \autoref{fig:main_fig}:
% 
\begin{align}
\feature^{(t+1)} &= \text{CrAtt}(\feature^{(t)}, \token^{(t)}) &\text{CrAtt}: \real^D \rightarrow \real^D
\\
\position, \confidence &= \text{MLP}(\feature^{(T)}; \pars_\text{MLP}) &\text{MLP}: \real^D \rightarrow \real^4
\end{align}
% 
where 
where $\text{CrAtt}(\feature, \token)$ is classical cross-attention~\cite{attention}:
% 
\begin{align}
\mathbf{Q} = \W_\mathbf{Q}^{(\iTokens)} \cdot \feature, \:\:
\mathbf{K} = \W_\mathbf{K}^{(\iTokens)} \cdot (w\token), \:\:
\mathbf{V} = \W_\mathbf{V}^{(\iTokens)} \cdot (w\token)
\\
\feature^{(t+1)} = \text{MLP}(\text{softmax}(\mathbf{Q} \cdot \mathbf{K}) \cdot \mathbf{V}; \pars_\text{MLP}^{(\iTokens)})
\end{align}
% 
and note that as we \textit{do not} share weights across cross-attention layers, hence the trainable parameters of our decoder are:
% 
\begin{align}
\pars_\decoder=[
\pars_\text{MLP},
\{\pars_\text{MLP}^{(\iTokens)}\},
\{\W_\mathbf{Q}^{(\iTokens)}\},
\{\W_\mathbf{K}^{(\iTokens)}\},
\{\W_\mathbf{V}^{(\iTokens)}\}]
\end{align}

\paragraph{Training}
At training time, we learn how to ``compress'' scenes into tokens, hence we need to train across a large collection of scenes:
% 
\begin{align}
\argmin_{\pars_\decoder, \{\scene_\iScenes\} } &\quad
\expect_\iScenes \:
\expect_\iImages \:
\expect_\iKeypoints
\quad
\loss{}(\keypoint^\iKeypoints; \scene_\iScenes, \pars_\decoder)
\\
\loss{}(\keypoint; \scene, \pars_\decoder) &= 
\hyper_\position \loss{$\position$} +
\hyper_\confidence \loss{$\confidence$} + 
\hyper_\text{L1} \loss{L1}
\\
\loss{$\position$} &= \Sigma_\iVoxel \: 
% \confidence_\iVoxel \cdot  \AT{WHY NOT? WEIRD}
\| (\position_v + \voxCenter_v) - \keypoint \|_1^1
\\
\loss{$\confidence$} &= \text{BCE}(\{ \confidence_\iVoxel \}, \{\keypoint \in  \voxel_v \})
\\
\loss{L1} &= \|w\|_1^1
\\
\position_\iVoxel, \confidence_\iVoxel &= \decoder(\Feature_i[\proj_\iImages(\keypoint)]; \tokens_v, \pars_\decoder)
\end{align}
\TODO{describe why we add $\voxCenter_v$, as we are doing local regression}
\TODO{here describe how the mini-batch is built (i.e. describe how the expectations are implemented) e.g. sampling one image from each voxel}

\TODO{2-stage training strategy. In the first training stage, training both the scaling factor $w$ and apply $L_{L1}$ loss. In the second training stage, we set the codes whose $w$ are less than a threshold to be 0 and finetune all the other codes.  We train the network with the sum of the coordinate regression loss $L_{c}$ and the binary cross entropy loss $L_{x}$.}

\paragraph{Scene adaption}
Given a new scene we'd like to localize within, we first fine tune the scene code $\scene$ using the input images and corresponding keypoints, while keeping $\pars_\decoder$ \textit{fixed}:
% 
\begin{align}
\argmin_{\scene} &\quad
\expect_\iImages \:
\expect_\iKeypoints
\quad
\loss{}(\keypoint^\iKeypoints; \scene, \pars_\decoder)
\end{align}
% 
which then allows to retrieve the dense coordinates of all pixels within a query image $\I$ via \eq{decoder}.
\TODO{does the L1 sparsity/pruning go here? it's only at inference time, not at training time, right?}
Note that the coordinate regression is performed per-voxel, as \eq{decoder} employs the codes of a \textit{particular} voxel; see~\autoref{fig:main_fig}.
Therefore, we... \TODO{and now stitch back in the filtering + PnP part here}

\paragraph{Inference}
\TODO{merge above}
Given a query image, we first retrieve top K most similar database images. Each database image $I_i$ covers a set of sub-regions $V_v$. The union of $V_v$ is represented as $\overline{V}$. Since the feature extractor is shared, we only extract image features once and predict the coordinates and confidences using the corresponding codes of each sub-region in $V_v$ respectively. We filter the points whose confidence score is lower than 0.5. All the remaining points are used to compute the camera pose with PnP algorithm combined with RANSAC.

\clearpage

\at{Our method encodes key-points with the 3D coordinates and visual features into a grid of latent codes.
% all the 3D coordinates with corresponding appearance features into latent codes.
For a query image, we regress the 3D coordinates for each keypoints by matching image features with those latent codes. The camera pose is computed by PnP algorithm combined with RANSAC using 3D coordinate predictions.}
\AT{this opening needs to be revised, no idea why you are telling me all of this}
The overview of our pipeline is shown in Fig. \ref{fig:main_fig}.

%\yasu{The structure and naming of this section, in particular, 3.2 and 3.3 seem a bit unnatural. We talk about scene division later without mentioning at all till 3.3? We should give a high level view of our system in the paragraph of Method, then explain each module one by one. Also, section 3 is an important section: Technical core. The first sentence can be ideally fancy. The current first sentence of section 3 is bad. Can you write a high level view of your system here (ideally with a cool sentence to start), then say that we first give preliminary, and explain these 2? modules..}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.3\textwidth]{image/transformer-temp.png}
%     \caption{Transformer block architecture. }
%     \label{fig:fig2}
% \end{figure}


\subsection{Data preparation}
Given a database of images $\{I_\iImages\}{\equiv}\{I_\iImages\}_{\iImages=0}^{\nImages}$ \AT{vote for using n=1...N, so I don't have to remember N is the endpoint of iterator i?} with known camera poses in a coordinate frame $\coordFrame$, visual localization aims to compute the camera pose $\qCamera$ corresponding to a query image $\qImage$.
\AT{who gives you $\coordFrame$?}

\paragraph{Pre-processing}
Following HLoc~\cite{sarlin2019coarse}, we first extract 2D keypoints from all the database images \AT{how many per image?}, and run COLMAP~\todocite{colmap} to triangulate 3D keypoints $\keypoints{=}\{\keypoint_\iKeypoints\}$ expressed in the coordinate frame $\coordFrame$.
\todo{During training, we predict the 3D coordinates of each keypoint conditioned on the input of database images, and these predictions are supervised by the 3D coordinates $P$.}
\AT{why is this important to mention here? drop or move}

% \mysubsubsection{Scene division}
\paragraph{Scene factorization}
% Previous dense regression methods~\cite{brachmann2017dsac} are only able to handle small scenes because the network capacity is limited.
\at{Due to limited network capacity, dense regression methods are only able to handle \textit{small} scenes; e.g.~\DSAC.}
% To overcome this issue, \ESAC divides a (large) scene into several sub-regions by clustering camera centers of database images and trains one network for each region.
\at{To overcome this issue, \ESAC factors a large scene into several sub-regions via camera clustering, and trains one regression network within \textit{each} region.}
% We adopt the same idea but differently, we divide the scene space into regular 3D grids of a fixed length. Specifically, given a set of coordinates $P$, we first compute the the range, $x$, $y$, $z$, of $P$ in all axis. Then, we evenly space $x$, $y$, $z$ with a fixed length $l$.
\at{Conversely, we take inspiration by recent progress in sparse 3D representations~\todocite{NSVF, iNGP}, factor large scenes via a regular grid with voxel size~$\gridEdgeLength$, ....}

\todo{Each grid in the scene space is considered as a sub-region.
For a specific sub-region, those points falling in that sub-region is regarded as the in-regions points, while all the other points is out-of-region points. We only keep the sub-region covered by at least 20 images. The image is regarded as covering some sub-region if it contain at least 20 in-region points. Each sub-region is assigned with a set of codes, where the coordinates, confidence score and visual descriptors of in-region points are injected. Besides, for each sub-region, we normalize the in-region coordinates with the their mean and use the normalized coordinates as ground truths. It is also noted that each image covers multiple sub-regions.}\AT{I'll rewrite}
\todo{To regress the coordinates of the whole image, one strategy is to concatenate all the codes from each sub-region and predict coordinates with one network forwarding. However, we find that those codes are hard to optimize under such settings. Therefore, our framework forwards image with different codes independently for each sub-region.}
\AT{this sounds like an ablation, move to results?}

\subsection{Key-point Coordinate regression with auto-transdecoder}
\todo{We introduce NeuMap architecture in this section. Our framework takes the input of images and predicts the coordinates of key-points with confidence scores through a transformer-based auto-decoder.}
\AT{move to 3.0}

\mysubsubsection{Feature extractor}
\todo{Dense coordinate regression~\cite{brachmann2017dsac, brachmann2019expert} is effective in handling small scale scenes. One drawback of those methods is that dense depth map is required in training stage. To handle scenes without dense depth map, ESAC~\cite{brachmann2019expert} supervises the dense coordinate predictions by a reprojection loss. However, the coordinate accuracy is far worse than supervised with ground truth coordinates. Therefore, our method predicts the coordinates of key-points, whose supervision can be obtained by database image matching and triangulation.}
\AT{this belongs to related works?}

Given an image $I_i$, we first extract its key-points $\mathbf{K_i}$. The key-point extractor can be any such as SIFT, Superpoint~\cite{detone2018superpoint}, r2d2~\cite{revaud2019r2d2}, and etc. We use r2d2 in implementation. We also extract a dense feature map $\mathbf{F^i}$ with CNN. Then, for each key-point in $\mathbf{K^i}$, we bilinearly interpolate the image features $\mathbf{F^{K_i}}$ from $\mathbf{F^i}$. Finally, we predict the coordinates along with their confidence scores of $\mathbf{K_i}$ with $\mathbf{F^{K_i}}$. %\ping{the symbols are confusing here. Typically, we use bold font for vectors and matrices. You might use a different font for sets.}

\mysubsubsection{Key-points confidence estimation} Given an image and latent codes of one specific sub-region, only the in-region points get supervision, so out-of-region points are inaccurate. Thus, those out-of-region points should not be used to compute camera poses. In addition to coordinate prediction, the network also outputs a confidence score for each key-point, indicating whether the prediction is in-region points. Specifically, we classify every key-point into in-region points or out-of-region points and use binary cross entropy to supervise the training.

\mysubsubsection{Auto-transdecoder} DeepSDF~\cite{park2019deepsdf} assigns one learnable code to each object. One shared MLP takes the concatenation of coordinates and the code to regress the signed distance. When applying this idea to coordinate regression, the most straightforward way is to concatenate $\mathbf{F^{K_i}}$ with one learnable code and regress the coordinates with a shared MLP. However, this method is successful in capturing simple object shapes, but unable to memorize the whole scene, since the capacity of one code is limited. Several transformer-based image matching works~\cite{sarlin2020superglue} applies cross attention between query and database image pairs. After each transformer block, the attention scores of matched descriptors become higher and the ambiguous matches become more distinct. In our framework, we encodes all the database images into latent codes. With similar spirit, we apply cross attention between the query image features $F^{K_i}$ and those $N$ codes. This computation graph is illustrated in Figure \ref{fig:main_fig}. Specifically, assuming $F^{K_i}$ is $F^{K_i}_0$, we compute the query $\mathbf{Q}$, key $\mathbf{K}$, and value $\mathbf{V}$ as follows:
\begin{align*}
    \mathbf{Q}&=\mathbf{W_q}\mathbf{F^{K_i}_j} \\
    \mathbf{K}&=\mathbf{W_k}\mathbf{T_j} \\
    \mathbf{V}&=\mathbf{W_v}\mathbf{T_j}\text{,}
\end{align*}
where $\mathbf{T_j}$ is the codes for transformer block $j$. Then, the output $\mathbf{F^{K_i}_{j+1}}$ is calculated as:
\begin{equation}
    \mathbf{F^{K_i}_{j+1}}=\text{MLP}(\text{softmax}(\mathbf{Q}\mathbf{K^T})\mathbf{V})
\end{equation}
We stack 6 transformer blocks to process image features and codes. Each block is assigned with a different set of $N$ codes $\mathbf{T_j}$ to increase the learning capacity. In the end, we regress the coordinates from the output of transformer blocks.



\subsection{Training}
We demonstrate the code pruning and training strategy in this section.

\mysubsubsection{Code pruning} Liu et al.~\cite{liu2017learning} shows that CNN is over-parameterized and channels can be pruned without loss of accuracy. The code-based representation also suffers from this issue, and we apply code pruning to remove redundant codes. Specifically, we multiply each code with a scaling factor $w_i$, and jointly train the codes with these scaling factors, with $L1$ loss imposed on $w_i$. After finishing training, we prune codes whose weights ($w_i$) are below a threshold \yasu{(See Sect.~\ref{section:experiments})}
% close to 0 
and fine-tune the remaining codes without $L_1$ loss.

\mysubsubsection{Training strategy} For each sub-region, the corresponding codes are trained with images that contain in-region points.
%
We first group all the training images into each sub-region set. During training, we randomly sample images from some region image set to optimize both the shared parameters and the corresponding codes supervised by the in-region points. However, random sample training images cause unstable gradients for codes, since the updating frequency of codes is different. Therefore, during each epoch, we sample 1 image from each sub-regions so all the codes are updated once. We adopt 2-stage training strategy. In the first training stage, we training both the scaling factor $W$ and apply $L1$ loss. In the second training stage, we set the codes whose $w_i$ are less than a threshold to be 0 and finetune all the other codes.  We train the network with the sum of the coordinate regression loss $L_{coords}$ and the binary cross entropy loss $L_{conf}$.
\begin{equation}
 L_{coords} = |C_{gt}-C_{pred}|,
\end{equation}
\begin{equation}
    L_{conf} = -(ylog(p)+(1-y)log(1-p)).
\end{equation}
The notation $C_{gt}$ is the ground truth coordinates, $C_{pred}$ is the predicted coordinates, $y$ is an indicator of in-region points, and $p$ is the confidence.


\subsection{Localization pipeline} Given a query image, we first retrieve top K most similar database images. Each database image $S_i$ covers a set of sub-regions $\mathbf{R_i}$. The union of $\mathbf{R_i}$ is represented as $\mathbf{R}$. Since the feature extractor is shared, we only extract image features once and predict the coordinates and confidences using the corresponding codes of each sub-region in $R$ respectively. We filter the points whose confidence score is lower than 0.5. All the remaining points are used to compute the camera pose with PnP algorithm combined with RANSAC.

==> tex_file/3_method_andrea.tex <==
\input{fig/overview.tex}
\section{Neural Coordinate Mapping}%Method}
% 
Given a scene represented by an image collection~$\{\I_\iImages\}{\equiv}\{\I_\iImages\}_{\iImages=0}^{\nImages}$ with camera calibrations $\{\camera_\iImages\}$ expressed in a (scene-specific) coordinate frame $\bar\camera$, we devise a technique that encodes the images into a \textit{compact} scene representation $\scene$.
We employ this scene representation to perform \textit{camera localization}, a task of predicting the camera $\camera$ of an image~$\I$ that was never seen before -- with a vantage point and/or appearance different from the one in the training dataset.
% 
We achieve this task by solving the proxy task of \textit{sparse coordinate regression}, where given a 2D keypoint~$\tilde\keypoint$ extracted from $\I$, we predict its corresponding 3D coordinate $\keypoint$~(\autoref{sec:regression}):
% 
\begin{align}
\keypoint = \decoder(\tilde\keypoint; \scene, \pars_\decoder)
\label{eq:scr}
\end{align}
% 
To supervise the process, the 2D keypoints are extracted from a pre-trained backbone~\todocite{r2d2}, and the corresponding ground-truth 3D keypoints are triangulated by photogrammetry~\todocite{colmap}~(\autoref{sec:training}):
% 
\begin{align}
\{\tilde\keypoint^\iKeypoints\} &= \keypointExtractor_\text{2D}(\I) % , \quad \forall \I \in \{\I_\iImages\}
&\text{(r2d2)}
\label{eq:r2d2}
\\
\{\keypoint^k\} &= \keypointExtractor_\text{3D}(\{\tilde\keypoint^k\}, \{\I_\iImages\})
&\text{(COLMAP)}
\label{eq:colmap}
\end{align}
% 
finally, we obtain camera localization by solving a perspective-n-point (PnP) problem~\todocite{pnp}~(\autoref{sec:inference}):
% 
\begin{align}
\camera = \text{PnP}(\{\keypoint^k\}, \{\tilde\keypoint^k\})
\end{align}


\subsection{Sparse feature regression}%\shitao{Sparse feature regression?}}
\label{sec:regression}
% 
% \paragraph{Keypoint featurization}
%We re-cast sparse coordinate regression as \textit{sparse feature regression}\shitao{Can we just call it sparse feature regression without mentioning sparse coordinate regression}.
Rather than directly mapping 2D pixels to 3D coordinates as in \eq{scr}, we compute the feature $\feature{\in}\real^\featureDim$ corresponding to a 2D keypoint $\tilde\keypoint$ with a trainable CNN backbone~$\featureBackbone$~\todocite{backbone}, and then regress 3D coordinates from this feature:
% 
\begin{align}
\keypoint = \decoder(\Feature[\tilde\keypoint]; \scene, \pars_\decoder), 
\:\: \Feature {=} \featureBackbone(\I; \pars_\featureBackbone)
\label{eq:sfr}
\end{align}

\paragraph{Voxelization}
We cache 3D keypoints of a scene in a \textit{sparse voxel grid} with voxels of uniform side length~$\gridEdgeLength$; see~\autoref{fig:overview}.
Denoting with $\odot$ the Hadamart (i.e., element-wise) product, we can formalize this as: \ping{I feel these three equations are unnecessarily complicated. It might be easier by just saying we divide the space into voxels of edge size $l$ and only keep those with 3D keypoints. The set of valid voxels is denoted as $\mathcal{V}$}
% 
\begin{align}
\{\voxCenter_\iVoxel\} &= \{ ( \mathbf{z} \odot \gridEdgeLength) \text{~~s.t.~~} \mathbf{z} \in \mathbb{Z}^3\}
&\text{(lattice)}
\\
\voxel_\iVoxel &= \{ \keypoint^\iKeypoints \text{~s.t.~} \| \voxCenter_\iVoxel - \keypoint^\iKeypoints \|_\infty \leq \gridEdgeLength \} 
&\text{(voxelize)}
\\
\voxel &= \{ \voxel_\iVoxel \text{~s.t.~} \voxel_\iVoxel \neq \emptyset \} 
&\text{(sparsify)}
\end{align}

\paragraph{Hybrid localized regression}
We voxelize space and solve a
% \textit{hybrid} 
classification-regression problem to boost performance: 1) Classifying whether a 2D keypoint belongs to a voxel and 2) Regressing its 3D position \textit{locally} within the voxel.
% As neural networks had originally been designed for classification tasks\shitao{Does it mean image classification}, 
%convert our regression problem into a \textit{hybrid} classification-regression problem:
% 
%\begin{itemize}
%\item we classify whether a 2D keypoint belongs to a voxel
%\item we regress its 3D position \textit{locally} within the voxel
%\end{itemize}
%
For this reason, we model our scene as a \textit{set} of latent codes $\scene {=} \{ \tokens_\iVoxel \}$ -- \textit{one per voxel} -- and modify~\eq{sfr} to reflect this design choice, where $f$ denotes the feature of a keypoint:
%\shitao{What is $f$? image features?}:
% 
\begin{align}
\tilde\decoder(\feature; \tokens_\iVoxel, \pars_\decoder) =
\begin{cases}
\position_\iVoxel &\text{(local position)}
\\
\confidence_\iVoxel &\text{(confidence)}
\end{cases}
\label{eq:hybrid-notsparse}
\end{align}
% 
\ping{is the feature $\ve{f}$ the same as the $\ve{F}[\tilde{\ve{k}}]$??}
The position in the scene coordinate frame $\bar\camera$ can be obtained as $\position_\iVoxel + \expect[\voxel_\iVoxel]$; that is, the local coordinate frame is centered at the mean of the keypoints falling within the voxel.
Additional details on the decoder architecture will be described in section~\autoref{sec:decoder}.

\paragraph{Sparsity}
To encourage learning of easy-to-compress representations, we promote sparsity in the learned scene codes by modulating the codes with a sparse matrix $\W$:
% 
\begin{align}
\decoder(\feature; \tokens_\iVoxel, \pars_\decoder) \equiv \tilde\decoder(\feature; \W \odot \tokens_\iVoxel, \pars_\decoder)
\label{eq:hybrid}
\end{align}

\subsection{Training}
\label{sec:training}
% 
At training time, we learn the weights of the feature encoder $\featureBackbone$, the decoder $\decoder$, and the \textit{compressed} scene representation for all training scenes~$\{\scene_\iScenes\}$ via generative latent optimization / auto-decoding ~\cite{park2019deepsdf}:
% 
\begin{align}
\argmin_{\pars_\featureBackbone, \pars_\decoder, \{\scene_\iScenes\}, \{\W_s\}}
\expect_\iScenes \: \expect_\iImages \: \expect_\iKeypoints \:\:
\loss{$\position$} + \loss{$\confidence$} +  \loss{L1}
\label{eq:training}
\end{align}
% 
% where in implementing $\expect_\iImages$ we ensure each mini-batch contains at least one image for every voxel.
\ping{We need to define what are the three terms $\mathbb{E}_s$, $\mathbb{E}_n$ and $\mathbb{E}_k$}The first loss is on sparse 3D keypoint regression:
% 
\begin{align}
\loss{$\position$} = \hyper_\position \cdot
\Sigma_\iVoxel \: 
(\keypoint^\iKeypoints \in \voxel_\iVoxel)
\cdot
\| (\position_\iVoxel + \expect[\voxel_\iVoxel]) - \keypoint^\iKeypoints \|_1^1
\end{align}
%
where $(\keypoint^\iKeypoints {\in} \voxel_\iVoxel) \in \{0,1\}$ is an indicator predicate that evaluates whether the keypoint belongs to the voxel in the training data.
The second classification loss (Binary Cross-Entropy) is on the confidence of a keypoint belonging to a particular voxel:
% via a classification loss (Binary Cross-Entropy):
% 
\begin{align}
\loss{$\confidence$} &= \hyper_\confidence \cdot \text{BCE}(\{ \confidence_\iVoxel \}, \{\keypoint \in  \voxel_\iVoxel \})
\end{align}
% 
The third loss enforces \textit{sparsity} and
%Finally, we enforce \textit{sparsity} in the representation via with the following loss to 
produces a \textit{compressed} representation:
% 
\begin{align}
\loss{L1} &= \hyper_\text{L1} \cdot \| \W_\iScenes \|_1^1
\end{align}

\paragraph{Training data}
As a source of supervision, we employ the 3D keypoints by \eq{colmap}, project them onto each training image, and bi-linearly interpolate the corresponding feature:
% 
\begin{align}
\feature^\iKeypoints_\iImages &= \mathbf{F}_\iImages[\proj_\iImages(\keypoint^\iKeypoints) ] , \:\: \mathbf{F}_\iImages {=} \featureBackbone(\I_\iImages; \pars_\featureBackbone)
\label{eq:decoder}
\end{align}
% 
$\proj_\iImages$ is a pinhole perspective projection constructed from camera extrinsics $\camera_\iImages$ plus fixed/known intrinsics.
With this, we can build our supervision triplet $(\position_\iVoxel, \confidence_\iVoxel, \keypoint)$:
% 
\begin{align}
\position_\iVoxel, \confidence_\iVoxel &= \decoder(\Feature_i[\proj_\iImages(\keypoint)]; \tokens_\iVoxel, \pars_\decoder)
\end{align}

\paragraph{Scene adaption}
Given a \textit{new} scene (i.e. not in the training data), we simply optimize the scene code $\scene$, while keeping $\pars_\decoder$ and $\pars_\featureBackbone$ \textit{fixed}:
% 
\begin{align}
\argmin_{\scene}
\: \expect_\iImages \: \expect_\iKeypoints \:\:
\loss{$\position$} + \loss{$\confidence$} +  \loss{L1}
\end{align}

\paragraph{Two-stage training}
Similarly to network pruning~\cite{liu2017learning}, we execute \eq{training} to convergence, set values of $\W_\iScenes$ that are below a certain threshold to zero, and fine-tune our model while keeping $\W_\iScenes$ frozen.

\subsection{Inference}
\label{sec:inference}
% 
Given a query image $\I$, we use an existing technique~\todocite{retrieval} to
% first 
retrieve the most similar database images \yasu{are there any key parameters to be used with this existing work/software}, which identifies a \textit{smaller} sparse subset of voxels~$\voxel{=}\{\voxel_\iVoxel\}_{\iVoxel=1}^\nVoxels$; see~\autoref{fig:overview}.
\AT{how are they identified? not described!!}
We then extract the set of~2D keypoints $\{\keypoint^\iKeypoints\}_{\iKeypoints=1}^\nKeypoints$ within $\I$ via~\eq{r2d2}, and for each of them regress their per-voxel confidence and positions via~\eq{hybrid}.
This generates a point cloud in $\real^{\nKeypoints \times \nVoxels}$, from which we discard points with confidence $\confidence{<}0.5$.
All the remaining points are used to compute the camera pose with PnP algorithm combined with RANSAC. \yasu{Do we use some software module for this? If so, just cite. If not, some information here? Maybe how many iterations to try. Any reference to a precise PnP solver, SVD based? Maybe rich's textbook again to cite?}
\AT{provide reference, how would I go to implement this if I were a poor brand new PhD student? combined how with RANSAC?}

\subsection{Decoder architecture}
\label{sec:decoder}
% 
Until now we simply denoted a (per-voxel) latent code as $\tokens$. In reality, this code is a \textit{set} of tokens.
Our decoder $\decoder(\feature; \tokens_\iVoxel, \pars_\decoder)$ is a set-decoder defined by the inductive relationship~(see \autoref{fig:overview}):
% 
\begin{align}
\feature^{(t+1)} &= \text{CrAtt}(\feature^{(\iTokens)}, \token^{(\iTokens)}) &\text{CrAtt}: \real^\dToken \rightarrow \real^\dToken
\\
\position, \confidence &= \text{MLP}(\feature^{(\nTokens)}; \pars_\text{MLP}) &\text{MLP}: \real^\dToken \rightarrow \real^4
\end{align}
% 
where $\feature^{(1)}{=}\feature$ and $\tokens_\iVoxel{=}\{\token_\iVoxel^{(\iTokens)} {\in} \real^\dToken\}_{\iTokens=1}^\nTokens$, and $\text{CrAtt}(\feature, \token)$ is classical cross-attention from transformers~\cite{attention}:
% 
\begin{align}
\mathbf{Q} = \W_\mathbf{Q}^{(\iTokens)} \cdot \feature, 
\mathbf{K} = \W_\mathbf{K}^{(\iTokens)} \cdot (\token), 
\mathbf{V} = \W_\mathbf{V}^{(\iTokens)} \cdot (\token)
\\
\feature^{(t+1)} = \text{MLP}(\text{softmax}(\mathbf{Q} \cdot \mathbf{K}) \cdot \mathbf{V}; \pars_\text{MLP}^{(\iTokens)})
\end{align}
% 
Since we \textit{do not} share weights across cross-attention layers, the trainable parameters are:
% 
\begin{align}
\pars_\decoder=[
\pars_\text{MLP},
\{\pars_\text{MLP}^{(\iTokens)}\},
\{\W_\mathbf{Q}^{(\iTokens)}\},
\{\W_\mathbf{K}^{(\iTokens)}\},
\{\W_\mathbf{V}^{(\iTokens)}\}]
\end{align}

==> tex_file/3_method_old.tex <==
\input{fig/overview.tex}
\section{Method}
% 
Given a scene represented by a set of reference images~$\{\I_n \}$ with known camera calibrations $\{\camera_n \}$ expressed in a (scene-specific) coordinate frame, we devise a technique that encodes these images into a \textit{compact} scene representation $\scene$.
We employ this scene representation to perform \textit{visual localization}, a task of predicting the camera $\camera_q$ of a query image~$\I_q$ that was never seen before -- with a vantage point and/or appearance different from the one in the reference image set.
% 



%Their corresponding 3D scene coordinates  $\{ \scenepoint_i \}$ are triangulated by COLMAP~(\autoref{sec:training}). It's noted that some of keypoints are not successfully triangulated, so their ground-truth 3D coordinates $\keypoint^k$ is empty. 


\subsection{Overview}
We achieve visual localization by solving the proxy task of \textit{scene coordinate regression} on \textit{sparse features}, where given a set of 2D key-point~$\{ \keypoint_i \}$ extracted from $\I_q$, we predict its corresponding 3D scene coordinate $\{ \scenepoint_i \}$~(\autoref{sec:regression}).
As shown in Figure~\ref{fig:overview}, our method extracts 2D key-points $\{ \keypoint_i \}$ following HLoc~\cite{sarlin2019coarse} with a pre-trained backbone, R2D2~\cite{revaud2019r2d2}. 
In order to determine their scene coordinates, we first compute a feature map 
%$\Feature$ 
of the image $\I_q$ with a trainable CNN backbone $\featureBackbone$, which is a ResNet18~\cite{he2016deep} and bilinearly interpolates the feature, and then solve the scene coordinate by a decoder $\decoder$ as,
%$\Feature(\keypoint_i)$ corresponding to a 2D keypoint $\keypoint_i$, and then regress 3D coordinates from this feature as,
% 
\begin{equation}
\scenepoint_i = \decoder(\featureBackbone(\I_q, \keypoint_i), \mathcal{S})
\label{eq:sfr}
\end{equation}
Here, $\mathcal{S}$ is the learned scene representation. Finally, we obtain camera localization by solving a perspective-n-point (PnP) problem~\cite{lepetit2009epnp}~(\autoref{sec:inference}) with 2D-3D correspondences from $\{ \keypoint_i \leftrightarrow \scenepoint_i \}$. 


\subsection{Sparse Scene Coordinate Regression}%\shitao{Sparse feature regression?}}
\label{sec:regression}



\paragraph{Scene Representation}
We first build a scene model to facilitate localization. Given a set of reference images, we extract 2D key-points by R2D2~\cite{revaud2019r2d2} and compute their corresponding 3D scene coordinates by COLMAP~(\autoref{sec:training}). Some of the key-points are not successfully triangulated, so their 3D coordinates are invalid. We cache 3D scene points in a \textit{sparse grid} with voxels of uniform side length~$\gridEdgeLength$ as shown in Figure~\ref{fig:overview}. 
We denote the $v$-th voxel as $\voxel_v$.
We then model the reference scene as a \textit{set} of latent codes $\scene {=} \{ \tokens_v \}$ -- \textit{one per voxel} -- and modify Equation~\ref{eq:sfr} to reflect this design choice as:
\begin{equation}
(\scenepoint^v_i, c^v_i) = \decoder(\featureBackbone(\I_q, \keypoint_i), \tokens_v)
\label{eq:hybrid-notsparse}
\end{equation}
Here, the scalar parameter $c^v_i$ is the confidence that the key-point $\keypoint_i$ is in the voxel $\voxel_v$, and $\scenepoint^v_i$ is the scene coordinate under the voxel attached coordinate frame, i.e., $\scenepoint_i = \scenepoint^v_i + \ve{O}_v$ and $\ve{O}_v$ is the mean of all the coordinates in $\voxel_v$. 

This formulation simultaneously solves a classification and regression problem: 1) classifying whether a 2D key-point belongs to a 3D voxel and 2) regressing its 3D position \textit{locally} within the voxel.
% 
%The position in the scene coordinate frame $\bar\camera$ can be obtained as $\position_\iVoxel + \expect[\voxel_\iVoxel]$; that is, the local coordinate frame is centered at the mean, $\expect[\voxel_\iVoxel]$, of the 3D coordinates falling within the voxel. 
%Additional details on the decoder architecture will be described in section~\autoref{sec:decoder}.

\paragraph{Sparsity}
Inspired by network pruning~\cite{liu2017learning}, we apply code pruning to remove redundant codes. Specifically, we multiply each voxel code in $\tokens_v$ with a scaling factor $w_v$, and jointly learn the codes with these scaling factors, with $L1$ loss imposed on $w_v$. After finishing training, we prune codes whose weights are below a threshold and finetune the remaining codes.

\paragraph{Scene Coordinate Regression}
\label{sec:decoder}
We use a set of per-voxel latent codes $\tokens_v$ to facilitate the learning of scene coordinate regression. 
The decoder $\mathcal{D}$ is a stacked transformer to regress the scene coordinates of the 2D image key-points. We include $T$ transformer blocks, (6 blocks in our implementation), defined by the inductive relationship~(see Figure ~\ref{fig:overview}) as,
\begin{align}
\feature_i^{(t+1)} &= \text{CrAtt}(\feature_i^t, \Tilde{\token}_v^t) \\
\Tilde{\token}_v^t &= w_v^t \token_v^t
\label{eq:attention}
\end{align}
where the feature $\feature_i^{(1)}{=}\featureBackbone(\I_q, \keypoint_i)$, $w_v^t$ is the scaling factor enforcing sparsity. Each transformer block contains a set of codes $\token_v^t$, and the final per voxel codes are~$\tokens_v {=} \{\token_v^t, 1 {\leq} t {\leq} T \}$.  The function $\text{CrAtt}(\cdot, \cdot)$ is classical cross-attention from transformers~\cite{attention}:
\begin{gather}
\mathbf{Q} = \W_\mathbf{Q}^{(\iTokens)} \cdot \feature^t_i, 
\mathbf{K} = \W_\mathbf{K}^{(\iTokens)} \cdot \Tilde{\token}_v^t, 
\mathbf{V} = \W_\mathbf{V}^{(\iTokens)} \cdot \Tilde{\token}_v^t
\label{eq:QKV}
\\
\feature^{(t+1)}_i = \text{MLP}(\text{softmax}(\mathbf{Q} \cdot \mathbf{K}) \cdot \mathbf{V})
\end{gather}
At the end of the stacked transformer, we apply another MLP to compute the scene coordinate and confidence as,
\begin{equation}
(\scenepoint^v_i, c^v_i) = \text{MLP}(\feature_i^{(T)})
\end{equation}


% 
%Since we do not share weights across cross-attention layers, the trainable parameters are:
% 
% \begin{align}
% \pars_\decoder=[
% \pars_\text{MLP},
% \{\pars_\text{MLP}^{(\iTokens)}\},
% \{\W_\mathbf{Q}^{(\iTokens)}\},
% \{\W_\mathbf{K}^{(\iTokens)}\},
% \{\W_\mathbf{V}^{(\iTokens)}\}]
% \end{align}

\subsection{Training}
\label{sec:training}
% 

At training time, we learn the weights of the feature encoder $\featureBackbone$, the decoder $\decoder$, and the \textit{compressed} scene representation for all training scenes~$\{\scene_\iScenes\}$ via generative latent optimization / auto-decoding ~\cite{park2019deepsdf} with the following loss:
% 
\begin{align}
\loss{} = \hyper_\position \cdot \loss{$\position$} + \hyper_\confidence \cdot \loss{$\confidence$} +  \hyper_\text{L1} \cdot \loss{L1}.
\label{eq:training}
\end{align}
We set the loss weights $\hyper_\text{x}$, $\hyper_\text{c}$, and $\hyper_\text{L1}$ to 1.

The scene coordinate loss is defined as,
\begin{equation}
\loss{$\position$} = 
\sum_v \sum_i \:\:
 (y_i^v) \cdot \| (\scenepoint^v_i + \ve{O}_v) - \scenepoint^*_i \|_2
\end{equation}
where $\scenepoint^*_i$ is the scene coordinate triangulated by COLMAP for key-point $\keypoint_i$, the binary variable $y_i^v$ indicates whether the triangulated scene coordinate $\scenepoint^*_i$ belongs to the voxel~$\voxel_v$. The key-points with no valid 3D coordinates (not successfully triangulated) do not belong to any voxel. 



The second term is a classification loss, i.e., a binary cross entropy, for the confidence $c_i^v$,
\begin{align}
\loss{$\confidence$} =  \sum_v\sum_i BCE(c^v_i, y^v_i) \end{align}

% 
The third term enforces \textit{sparsity} and produces a \textit{compressed} representation, which is defined as,
\begin{align}
\loss{L1} &=  \sum_{v} \sum_{t=1}^T \| w_v^t \|_1,
\end{align}
where $w_v^t$ is the sparsity factor in Equation~\ref{eq:attention}.


\paragraph{Training strategy}
We learn the decoder $\decoder$, the CNN backbone $\featureBackbone$, and the scene representation $\scene$ with voxel sampling. At each iteration, we randomly choose $B$ voxels, where $B$ is the batch size. Each voxel $\voxel_v$ has a set of reference images $\ve{I}_v$, each of which contains at least 20 scene points in $\voxel_v$. We then sample one training image for each voxel and optimize $\decoder$, $\featureBackbone$, and the scene codes of sampled voxels by minimizing the training loss in Equation~\ref{eq:training}. We sample voxels without replacement, so all scene codes are updated once at each epoch.

Similarly to network pruning~\cite{liu2017learning}, we minimize the training loss to convergence, set sparsity factors $w_v^t$ whose values are below a certain threshold to zero, and fine-tune our model while keeping $w_v^t$ frozen.

% 
% \begin{align}
% \feature^\iKeypoints_\iImages &= \mathbf{F}_\iImages[\proj_\iImages(\keypoint^\iKeypoints) ] , \:\: \mathbf{F}_\iImages {=} \featureBackbone(\I_\iImages; \pars_\featureBackbone)
% \label{eq:decoder}
% \end{align}
% 


% With this, we can build our supervision triplet $(\position_\iVoxel, \confidence_\iVoxel, \keypoint)$:
% % 
% \begin{align}
% \position_\iVoxel, \confidence_\iVoxel &= \decoder(\Feature_i[\proj_\iImages(\keypoint)]; \tokens_\iVoxel, \pars_\decoder)
% \end{align}

\paragraph{Scene adaption}
Given a \textit{new} scene (i.e., not in the training data), we simply optimize the scene code $\scene$, while keeping decoder $\decoder$ and CNN backbone $\featureBackbone$ \textit{fixed}. In this way, our scene representation $\scene$ is scene specific, but the decoder $\decoder$ and feature extractor $\featureBackbone$ are scene agnostic. 
% 
% \begin{align}
% \argmin_{\scene}
% \: \expect_\iImages \: \expect_\iKeypoints \:\:
% \loss{$\position$} + \loss{$\confidence$} +  \loss{L1}
% \end{align}


\subsection{Inference}
\label{sec:inference}
% 
Given a query image $\I_q$, we use an existing deep image retrieval method~\cite{revaud2019learning, arandjelovic2016netvlad} to retrieve the most similar reference images, which activate a subset of voxels; see Figure~\ref{fig:overview}. A voxel $\voxel_v$ is activated if one of the retrieved reference images contains at least 20 scene points in $\voxel_v$. For large-scale scenes, we typically get around 100-200 voxels, while for small-scale scenes, we consider all the voxels without image retrieval. 
We then extract a set of 2D key-points $\{\keypoint_i \}$ within $\I_q$, and for each of them, regress their per-voxel confidence and positions via Equation~\ref{eq:hybrid-notsparse}.
%This generates a point cloud in $\real^{\nKeypoints \times \nVoxels}$, 
We discard points with confidence $\confidence{<}0.5$. All the remaining points are used to compute the camera pose with the PnP algorithm combined with RANSAC, implemented in Pycolmap~\cite{pycolmap2022}.
%\yasu{Do we use some software module for this? If so, just cite. If not, some information here? Maybe how many iterations to try. Any reference to a precise PnP solver, SVD based? Maybe rich's textbook again to cite?}
%\AT{provide reference, how would I go to implement this if I were a poor brand new PhD student? combined how with RANSAC?}
%\yasu{I thought that }



==> tex_file/4_experiments_old.tex <==
\section{Experiments} \label{section:experiments}
We conduct extensive evaluations with twelve competing methods on five benchmarks.
%on various datasets to show the effectiveness of our method.

\begin{figure*}
    \centering
    \small
    \includegraphics[width=0.95\textwidth]{image/dataset_vis.pdf}
    \caption{Sample images from 7scenes, ScanNet, Cambridge, Aachen Day $\&$ Night, and NAVER LABS datasets.}
    \label{fig:dataset}
\end{figure*}

\subsection{Datasets}
We use 7scenes~\cite{shotton2013scene}, Cambridge landmarks~\cite{kendall2015posenet}, Aachen Day $\&$ Night~\cite{sattler2012image}, NAVER LABS datasets~\cite{lee2021large}, and ScanNet~\cite{dai2017scannet} (See Fig.~\ref{fig:dataset}). For 7scenes, Cambridge, Aachen, and ScanNet, we train a separate model for each dataset. Within each dataset, all the scenes share the same network parameters. For NAVER, we train one model for one scene because the codes for the scene are too large to fit in GPU memories.
%could not load all the codes in GPU memories. 
%
% how to train
In addition, for 7scenes, Cambridge, and NAVER, we train models from scratch. For Aachen, whose images have high view/illumination differences, we use a feature extractor from LoFTR~\cite{sun2021loftr}, which was pretrained with images containing such variations.
% trained with is robust against appearance variations.
%to initialize the feature extractor, since Aachen images have high appearance variations (i.e., nights and days)
%the database images in Aachen
%and are not enough for training a robust model.
ScanNet is not a standard localization dataset but is similar to 7scenes. To illustrate our scene-agnostic network and scene-specific code design, we use 80 scenes to train the scene-agnostic network and fine-tune the codes on 1 scene (scene0708) for ScanNet.
%
% code pruning
We demonstrate code pruning for 7scenes, Cambridge, and Aachen, where the pruning threshold is 0.00003, 0.05, and 0.2, respectively. We use median translation/rotation errors to evaluate 7scenes, Cambridge, and ScanNet. For Aachen and NAVER, the accuracy under different thresholds is the standard metric used.

\subsection{Implementation details} We use ResNet-18~\cite{he2016deep} to extract image features and train models with 8 V100 GPUs with a batch size of 256. We set the initial learning rate to 0.002 to train the scene-agnostic parameters and 0.0001 to train the scene-specific codes. After every 30 epochs, we multiply the learning rate by 0.5. We train the model for 200 epochs in the first stage and fine-tune the model for 100 epochs in the second stage. For training data generation, we use r2d2~\cite{revaud2019r2d2} to extract key-points and run triangulation to get coordinates in Cambridge, Aachen, and NAVER. We use depth images to obtain 3D coordinates in 7scenes and ScanNet.


\subsection{Main results with code-pruning}
We show the results after code-pruning for 7scenes, Cambridge, and Aachen datasets.
%Day $\&$ Night, Cambridge, and 7scenes datasets.

\input{table/Aachen_table}
\input{table/7scene_table}
\input{table/cambridge_table}
\paragraph{Aachen Day $\&$ Night}
Table ~\ref{tab:aachen} compares NeuMap with other methods in this large-scale outdoor dataset. We implement three versions of NeuMap by varying the size of voxels (either 8 or 10 meters) with or without code-pruning.
%: (Ours (8m, 100)) The scene is divided into sub-regions of 8 meters in length with code-pruning; and (Ours (8m,
%and code pruning is not applied, denoted as \emph{ours (8m, *)} and 2) the scene is divided into sub-regions of 10 meters' length and code pruning is applied, denoted as \emph{Ours (10m, *)}.
%
The version with 8 meters without code-pruning serves as the performance upper-bound.


Existing coordinate regression methods (i.e., ESAC or DSAC++) perform badly in this dataset. DSAC++ cannot fit the whole scene into a single network. ESAC is not robust to view and illumination differences. NeuMap is the first coordinate regression method with competitive results in large-scale outdoor datasets. NeuMap also outperforms another non-feature matching-based method, PixLoc, by a large margin. Cascaded~\cite{cheng2019cascaded}, QP+R.Sift~\cite{mera2020efficient} and Squeezer~\cite{yang2022scenesqueezer} are scene compression methods based on feature matching. NeuMap outperforms Cascaded and QP+R.Sift by a large margin. Both methods utilize numeric quantization for compression (converting 32-bit floats to 8-bit integers), which is orthogonal to our scheme and would likely boost our performance further once combined.
%It is noted that both of methods utilize quantization to convert 32-bit floats to 8-bit integers, which is orthogonal to our method. 



Squeezer~\cite{yang2022scenesqueezer} is built on HLoc~\cite{sarlin2019coarse}, which extracts and matches key-points by superpoint~\cite{detone2018superpoint} and superglue~\cite{sarlin2020superglue}. Squeezer removes redundant key-points by solving quadratic programming and achieves impression compression at the expense of performance. We use superpoint~\cite{detone2018superpoint} features (float32) for Squeezer. The NeuMap with code pruning (10 meters) achieves similar performance as Squeezer at 70 Megabytes smaller representation size. Even at extremely high compression ratios, NeuMap obtains good results, where the total mapping size is only 6 Megabytes. Squeezer fails at such ratios as in Fig.~\ref{fig:teaser}.


\paragraph{Cambridge} 
Table ~\ref{tab:cambridge} compares performance for Cambridge. We use triangulated points for supervision and divide each scene into voxels of 200 meters in length. NeuMap achieves similar performance as DSAC++ at 100 to 1000 times smaller representation size.
%
%Basically, we obtain the similar performance as DSAC++, but with much smaller scene representation size, achieving 100-1000 compression ratio.
NeuMap outperforms Squeezer by a large margin, this time, in terms of both accuracy and scene representation size.
%Besides, we also outperform the state-of-the-art scene compression method Squeezer~\cite{yang2022scenesqueezer} by a large margin in terms of both scene representation size and errors. 
%In contrast, our method achieve very small mapping size without accuracy loss. It is noted 
Our compression design is simple (i.e., latent codes with auto-transdecoder) compared to Squeezer, which has a complex pipeline.
%that we don't design a super complex compression pipeline as Squeezer. The idea of storing all mapping information into codes implicitly has a natural advantage of the scene representation size.

\paragraph{7scenes} Table ~\ref{tab:7scenes} shows the results, where we use depth images for supervision and train models from scratch. A scene is divided into voxels of 3 meters in length. NeuMap achieves the same performance as DSAC++, HLoc, and DSM with a 200-1000 times smaller data size.
%We can see our performance is the same as DSAC++, HLoc, DSM, but with much smaller representation size of over 200X times the compression ratio. 

\subsection{Main results without code-pruning}

\input{table/nl_table}
NAVER is a large-scale indoor localization dataset. Each scene contains roughly 20,000 images. We use 3 scenes (Dept. B1), (Dept. 1F), and (Dept. 4F) for experiments. We divide each scene into voxels of 4 meters in length, which results in approximately 2,000 voxels, and assign $50\times 6$ codes to each voxel, and train a model from scratch without code pruning. Table ~\ref{table:naver} compares NeuMap against three methods. Each method is trained with "training images" and evaluated with "validation images" of their dataset. NeuMap outperforms a state-of-the-art coordinate regression method ESAC by a large margin with a much smaller representation size. In comparison to feature matching methods (D2Net and R2D2), NeuMap has similar accuracy when the error thresholds are (0.25m, 2$^{\circ}$) and (1m, 5$^{\circ}$), while the representation size is 200 times more compact even without code pruning.
%However, we still achieve over 200$\times$ compression even without code pruning. The performance can be further improved if engineer efforts and computation resources are spent on this dataset.

\subsection{Evaluating code fine-tuning}

\input{table/scannet_table}
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{image/attn-score-vis.png}
    \caption{Attention score visualization. We choose one specific code, compute the attention scores for all pixels, and visualize scores by normalizing all the pixels. Each row is the visualization results for the same code. We can see that each code memorizes a specific area. } \label{fig:attn_score}
%\vspace{-1em}
\end{figure*}
Our scene-agnostic network and scene-specific code design allows us to fine-tune only the codes for a new scene while fixing the network weights. We use the ScanNet dataset for experiments. We train NeuMap with 1, 10, 20, 40, or 80 scenes and choose 1 new testing scene for fine-tuning and evaluation. For each scene, we randomly sample 10\% of the frames for testing, while the rest becomes the training set.
Figure ~\ref{fig:scannet} shows the median translation and the median rotation errors for the fully-trained (i.e., optimizing both network weights and codes) and the fine-tuned NeuMap models. The fully-trained models' accuracy does not drop as the number of training scenes increases, showing that NeuMap handles an arbitrary number of scenes without a performance drop. On the other hand, fine-tuned models improve accuracy as more training scenes are used to learn a generalizable scene-agnostic network.
%On the other hand, we can see that the testing errors is reduced when training the network with more training scenes, which demonstrates that the generalization ability is enhanced. This experiment also illustrates that the scene agnostic CNN and transformer is fully decoupled with scene specific latent codes. Our model can memorize infinite number of scenes by storing mapping information into codes. 



\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{image/rebuttal_heatmap_compress.png}
    \caption{Visualization of activated regions. Deep blue delineates more codes, while orange corresponds to fewer codes.}
    \label{fig:vis}
\end{figure}

\subsection{Ablation studies and visualization}

We conduct several ablation studies and show visualization results for NeuMap.

\input{table/code_table}
\paragraph{Code number and code-pruning} 
Table ~\ref{tab:code} shows how the number of codes influences the accuracy of Aachen Day $\&$ Night dataset. NeuMap obtains good results even with 1 code, while the performance improves as we add more codes. The table also shows the results of code pruning, which reduces the number of codes from 100 to 25 on average while maintaining similar accuracy. The pruned version with 25 codes is far superior to the counterpart without pruning which was trained with 25 codes from the start.
%We show the results of code pruning on Aachen Day $\&$ Night dataset. The code pruning can reduce the codes from 100 to 25 while maintaining the similar accuracy. Compared with the counterpart trained with the same number of codes, code pruning is able to obtain much better performance.

\input{table/block_table}

\paragraph{Attention score visualization} Figure ~\ref{fig:attn_score} shows the attention scores between one code and image features in different views. The score for pixel $i$ and code $j$ is computed as
\begin{align}
    s_i^j = [\text{softmax}(\mathbf{Q} \cdot \mathbf{K})]^j.
\end{align}
$[.]^j$ is the $j^{th}$ element of the vector. $\mathbf{Q}$, $\mathbf{K}$ is the same as Equation \ref{eq:QKV}. We normalize the scores across an image by
\begin{align}
    \Tilde{s}_i^j=\frac{((s_i^j)-a)}{a-b}.
\end{align}
$a$ and $b$ are the minimum and maximum values in an image. A code activates and stores information for a consistent set of pixels corresponding to the same 3D scene structures.
%of different views for the same code in . We can see that for the same code, the same area is activated. This indicating that each code is able to memorize a specific area. 

\paragraph{Transformer block number} Table ~\ref{tab:block_num} shows the results under different transformer block numbers. The performance improves as we use more transformer blocks.


